Exact and Approximate Heterogeneous Bayesian Decentralized Data Fusion

In Bayesian peer-to-peer decentralized data fusion, the underlying distributions held locally by autonomous agents are frequently assumed to be over the same set of variables (homogeneous). This requires each agent to process and communicate the full global joint distribution, and thus leads to high computation and communication costs irrespective of relevancy to specific local objectives. This work formulates and studies heterogeneous decentralized fusion problems, defined as the set of problems in which either the communicated or the processed distributions describe different, but overlapping, random states of interest that are subsets of a larger full global joint state. We exploit the conditional independence structure of such problems and provide a rigorous derivation of novel exact and approximate conditionally factorized heterogeneous fusion rules. We further develop a new version of the homogeneous Channel Filter algorithm to enable conservative heterogeneous fusion for smoothing and filtering scenarios in dynamic problems. Numerical examples show more than $99.5\%$ potential communication reduction for heterogeneous channel filter fusion, and a multi-target tracking simulation shows that these methods provide consistent estimates while remaining computationally scalable.

==> Text/FactorAlgorithms.tex <==
In section \ref{sec:factorCF} we derived equations that form the basis of the conditionally factorized CF family of algorithms. In this section use Factor graphs to develop the algorithms for heterogeneous decentralized data fusion. To get insight and be able to track the common information explicitly we first consider linear Gaussian distributions and use the iFactor version of the factor graph. Since assumptions regarding conditional independence requires different treatment in the static vs dynamic cases, we will analyze the static case first.   
\subsection{Static Problems}

We start our analysis before the first measurement and fusion step, and look at the local graph of agent \emph{i}.
There are three main steps performed on the graph, in the brackets we see the local distribution represented by the graph:
\begin{enumerate}
    \item \textbf{Fuse local measurements} = add measurement factors to the graph - $p_i(x,s_i|m_i^1,y_i^1)$.
    \item \textbf{Prepare local message} = add \emph{anti-factor} and refactor graph - $p_i(x,s_i|m_i^1,y_i^1)=p_i(x|m_i^1,y_i^1)\cdot p_i(s_i|x,m_i^1,y_i^1)$.
    \item \textbf{Fuse} = add all received fusion factors to the graph - $p_i(x,s_i|m_i^1,y_i^1,m_j^1,y_j^1)$.
\end{enumerate}
The term \emph{anti-factor} was introduced in \cite{cunningham_ddf-sam_2013} as a mean to remove information in a graph-SLAM algorithm. Similarly we use it here to account for implicit common information by subtracting it before marginalization.

\od{Add figure that show graphs}

\subsection{Dynamic Problems}
A dynamic fusion problem can be divided into two sub-problems: (i) full time history estimate, i.e. without marginalization of past states in the local estimation step, as common in SLAM problems where robot past pose states are kept (ii) sliding window estimate, where there is a marginalization of past states, as done in Kalman filtering (for a sliding window of 1). As will be shown, in heterogeneous fusion, local marginalization of past states leads to implicit common information not tracked by the channel filter and results double counting. 
We start with analyzing problem (i) and than show the challenge that arise due to marginalization and offer an approximate conservative marginalization step to be able to separate the implicit and explicit common information and avoid double counting.

There are two main technical insights that enable the tracking of common information in a dynamical problems and allow marginalization. First, we look at what happens in the prediction step and how it is translated to the iFactor graph.\\
The augmented state (AS) filter \cite{chong_comparison_2014} estimates the distribution of the joint state $x_{k:n|k}=[x_{k|k}^T,...,x_{n|k}^T]^T$, accumulated over a time window from initial time $t_n$ up to the present time $t_k$. 
The prediction step in ref.\cite{chong_comparison_2014} is given in state space. We present an information space version of it and name it \emph{iAS}.
The predicted information matrix and vector are given by: 
\begin{equation}
    \begin{split}
       \Lambda_{k:n|k-1}&=
       \begin{pmatrix} Q^{-1} & -Q^{-1}\mathbf{F}  \\
       -\mathbf{F}^TQ^{-1}  & \Lambda_{k-1:n|k-1}+\mathbf{F}^TQ^{-1}\mathbf{F}
        \end{pmatrix},\\
       \zeta_{k:n|k-1}&=
       \begin{pmatrix}Q^{-1}Gu_k \\ 
       \zeta_{k-1:n|k-1}-\mathbf{F}^TQ^{-1}Gu_k\end{pmatrix},
   \end{split}
    \label{eq:iAS_pred_Final}
\end{equation}
where $\mathbf{F}=\big[F_{k-1} \ \ 0_{m \times m(k-n-2)} \big ]$ and $m$ is the size of the (not augmented) state vector. \\
The main insight from (\ref{eq:iAS_pred_Final}) is that the predicted state information block $\Lambda_{k|k-1}=Q^{-1}$ (left upper block in $\Lambda_{k:n|k-1}$) does not have terms relating past information states (and similarly in the information vector), i.e. it can be separated in an additive manner. The predicted information matrix can be expressed as a summary of three factors: 
\begin{equation}
    \begin{split}
       \Lambda_{k:n|k-1}&=\overbrace{
       \begin{pmatrix} Q^{-1} & 0  \\
       0  & 0
        \end{pmatrix}}^{f(x_k)}
        +\overbrace{\begin{pmatrix} 0 & -Q^{-1}\mathbf{F}  \\
       -\mathbf{F}^TQ^{-1}  & 0
        \end{pmatrix}}^{f(x_k|x_{k-1}:n)}\\
        &+\underbrace{\begin{pmatrix}0 & 0  \\
       0 & \Lambda_{k-1:n|k-1}+\mathbf{F}^TQ^{-1}\mathbf{F}
        \end{pmatrix}}_{f(x_{k-1}:n)},
    \end{split}
    \label{eq:iAS_pred_Final}
\end{equation}
where here we omit the information vector from the factor notation for abbreviation.
\od{need to reference a graph}\\
As will be demonstrated, in order to be able to track common information, 
it is of interest to perform approximate conservative marginalization. We first state fact $10.11.18$ from \cite{bernstein_scalar_2018} about two positive-definite (PD) matrices $A,B$:
\begin{equation}
    (A+B)^{-1}\leq \frac{1}{4}(A^{-1}+B^{-1}),
    \label{eq:inverseInequality}
\end{equation} 
where equality holds when $A=B$.  
For a series of PD matrices $A_1...A_n$ we can recursively use eq. (\ref{eq:inverseInequality}) to get:
\begin{equation}
    (A_1+A_2+...+A_n)^{-1}\leq \sum_{i=1}^{n}\frac{1}{4^i}A_i^{-1}
    \label{eq:inverseInequality}
\end{equation} 
The second insight then results from this equation, where a marginalization of a past variable requires taking the inverse of two kind of factors connected to this variable, local factor and common factor. The local factor includes implicit common information that is not tracked by the channel filter and will be coupled to the common factor by taking the inverse. Using this approximation we are able to keep the two factors separated in a conservative way.\\
\od{need to reference a graph}
